ESTER: A Machine Reading Comprehension Dataset for Event Semantic Relation Reasoning

Understanding how events are semantically related to each other is the essence of reading comprehension. Recent event-centric reading comprehension datasets focus mostly on event arguments or temporal relations. While these tasks partially evaluate machines' ability of narrative understanding, human-like reading comprehension requires the capability to process event-based information beyond arguments and temporal reasoning. For example, to understand causality between events, we need to infer motivation or purpose; to establish event hierarchy, we need to understand the composition of events. To facilitate these tasks, we introduce ESTER, a comprehensive machine reading comprehension (MRC) dataset for Event Semantic Relation Reasoning. The dataset leverages natural language queries to reason about the five most common event semantic relations, provides more than 6K questions and captures 10.1K event relation pairs. Experimental results show that the current SOTA systems achieve 22.1%, 63.3%, and 83.5% for token-based exact-match, F1, and event-based HIT@1 scores, which are all significantly below human performances (36.0%, 79.6%, 100% respectively), highlighting our dataset as a challenging benchmark.

==> 08-discussion.tex <==
\section{Discussion}
\label{sec:discuss}
\mypar{Learning with Partial Signals.} In Table~\ref{tab:ans-num}, we show that the validated data contain about 0.5 more answers per question. \textbf{Proximity} and \textbf{saliency} are the two reasons we observe that contribute most to this discrepancy. Our input data include long passages with an average of 128 tokens. Even a well-trained worker can overlook relations for event pairs that are physically distant from each other. Moreover, long-distance relations are often less salient. For non-salient event relations, expert or external knowledge may be needed to disambiguate. We found workers tend to be conservative by avoiding using these non-salient relations as answers.

\begin{table}[htbp!]
\centering
\scalebox{0.8}{
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|cccc}
\toprule
& \#Ans. & $F_1^E$ & $F_1^T$ & \textbf{HIT@1}\\
\midrule
original & 1.41 & 56.6($\pm$0.5) & 53.0($\pm$0.3) & 72.7($\pm$0.6) \\
completed & 1.84 & 56.7($\pm$0.5) & 52.7($\pm$0.3) & 72.5($\pm$0.8) \\
\bottomrule
\end{tabular}
}
\caption{Performances on test data. Workers' original annotations v.s. completed by another worker.}
\label{tab:completed-samples}
\end{table}

However, when presented with enough examples comprising of both complete and partial answers, human beings can learn, generalize and thus find complete answers for unseen questions. Learning from partial annotations has been widely explored in several tasks such as named-entity recognition \citep{huang2019learning, shang2018learning}, word segmentation, and part-of-speech tagging \citep{tsuboi-etal-2008-training, yang-vozila-2014-semi}. Therefore, an encouraging future research direction of creatively using our data would be either leveraging or advancing partial signal learning methods in order to close the gap between SOTA models and human performances as shown in Table~\ref{tab:results-answer-gen}.
